Study of the symmetry of electronic system of the Weyl semimetal GdBiPt using rotational anisotropy of second harmonic generation

The half-Heusler compound GdBiPt orders antiferromagnetically around $T_\mathrm{N}=8.5$ K which implies breaking the time reversal symmetry as well as the translational symmetry. This combination preserves the global symmetry. Here, we used rotational anisotropy of second harmonic generation (SHG) to study the symmetry changes associated with this phase transition. GdBiPt crystallizes in the space group $F\overline{4}3m$, which does not change through the phase transition. From powder neutron diffraction, the proposed magnetic point group for the magnetic unit cell is $3m$. We carried out a symmetry analysis of the SHG patterns. Above \tn, the SHG data shows a $C_2$ symmetry which excludes the point group $\overline{4}3m$, as well as the $3m$ point group which represents a $[1 1 1]$ facet of the sample. Thus, we considered the point groups $2$ and $m$, but we have to reject the first one as the associated tensor elements poorly represent the angular dependence SHG. Finally, a superposition consisting of the point groups $3m$ and $m$ fit the data correctly. Below \tn, we had to add a third contribution associated with magnetic points group $m'$ in order to properly describe the SHG signal. The SHG intensity is linearly proportional to the antiferromagnetic order parameter. This allows us to determine $T_\mathrm{N}=9.61\pm0.48$ K and a critical exponent $\beta=0.346\pm0.017$, which are in agreement with the values found in the literature.

==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

